Robust 360-8PA: Redesigning The Normalized 8-point Algorithm for 360-FoV Images

This paper presents a novel preconditioning strategy for the classic 8-point algorithm (8-PA) for estimating an essential matrix from 360-FoV images (i.e., equirectangular images) in spherical projection. To alleviate the effect of uneven key-feature distributions and outlier correspondences, which can potentially decrease the accuracy of an essential matrix, our method optimizes a non-rigid transformation to deform a spherical camera into a new spatial domain, defining a new constraint and a more robust and accurate solution for an essential matrix. Through several experiments using random synthetic points, 360-FoV, and fish-eye images, we demonstrate that our normalization can increase the camera pose accuracy by about 20% without significantly overhead the computation time. In addition, we present further benefits of our method through both a constant weighted least-square optimization that improves further the well known Gold Standard Method (GSM) (i.e., the non-linear optimization by using epipolar errors); and a relaxation of the number of RANSAC iterations, both showing that our normalization outcomes a more reliable, robust, and accurate solution.

==> 1_0_intro.tex <==
\section{Introduction}\label{sec:sec_intro_test}

Estimating the relative pose between cameras has been studied for years in computer vision and robotics. For instance, Visual Odometry (VO) and Simultaneous Localization and Mapping (SLAM) take the sequence of images as inputs and infer the camera pose of each keyframe. As 360-FoV cameras have become widespread in recent years, incorporating omnidirectional views into VO/SLAM becomes more popular.~However, most of the existing approaches for a reliable camera pose solution, mainly aim at perspective projection.

Several well-known SLAM and Structure-from-Motion (SfM) algorithms~(e.g. \cite{mur2015orbslam, openvslam2019,openmvg_moulon2016, GuanSfM_VMF, pagani2011_sfm_some_loss_func}) rely on an estimated essential matrix to remove outliers of all correspondences across images, which not only provides a reliable initialization for the relative pose estimation but also stabilizes camera re-localization results in VO~(e.g. \cite{scaramuzza2011tutoI, hartleyBoock2003}). In practice, the procedure of calculating essential matrix includes two main steps: 1) An abundant number of salient points, i.e., \textit{key-features}, are extracted from each image, followed by matching them across different views; 2) An essential matrix is calculated to satisfy the epipolar constraints built upon the correspondences. After the essential matrix is derived, the relative camera pose can be recovered by singular value decomposition~(e.g.  ~\cite{scaramuzza2011tutoI, hartleyBoock2003}).

\input{figures_src/teaser}

To solve the essential matrix, several classic approaches have been proposed. 
For instance, the five-point (5-PA)~\cite{nister2004efficient} and eight-point (8-PA)~\cite{higgins1981computer} algorithms are commonly adopted in many SLAM/SfM systems.
However, although 5-PA comes in handy for solving the essential matrix, most of the implementations are deployed for perspective cameras and their formulation usually involves multiple ambiguous results.
In contrast, 8-PA solves the essential matrix with a linear system without the ambiguity as to the 5-PA. Moreover, due to its stability for wide field-of-view (FoV) cameras, 8-PA is extensively used for spherical projection~(e.g. \cite{GuanSfM_VMF,openmvg_moulon2016, openvslam2019, fermuller1998spherical_SFM,fujiki2007epipolar,taira2015robust_features}). However, as more correspondences are needed to solve the essential matrix in 8-PA, a higher computational cost is also required in the outlier removal procedure (e.g., RANSAC \cite{RANSAC_fischler1981random}).

Although studies~\cite{da2019perturbation} show that a wider FoV may increase the stability of 8-PA for spherical cameras, this assumes that matched key-points in the image are well-distributed in the whole FoV. However, in practice, the distribution mainly depends on external factors, which sometimes yields to clustered key-feature groups (see Fig. \ref{fig:teaser}), resulting in a reduction in the use of the wide FoV~(e.g. \cite{book_ma2012invitation, rublee2011orb_features,taira2015robust_features}).
In this work, we improve the 8-PA~\cite{higgins1981computer} for spherical cameras by re-defining \textit{the pre-conditioning} strategy proposed by~\cite{hartley1997defense} to be applied to spherical projection, which effectively deals with outliers and uneven key-feature distributions for 360-FoV images.
Moreover, we extend the usage of our novel pre-conditioning by proposing a constant weighted least-square solution, which improves the Gold Standard Method (GSM)~\cite{pagani2011_sfm_some_loss_func} that is used to refine the camera pose. Both approaches aim to evaluates a robust estimation of an essential matrix, without much impact on computation time.

We evaluate our methods under both sequences of real 360-FoV and fish-eye scenarios, where the former is our own dataset, collected from Matterport3D~\cite{Matterport3D} and rendered using MINOS~\cite{minos2017}, while the latter is the TUM-VI dataset~\cite{TUMVIschubert2018dataset}. We show that our method significantly outperforms the state-of-the-art 8-PA for spherical cameras without the overhead in computation time, demonstrating the robustness of our method against noise and outliers.
In favor of the research community, we will make our dataset (namely 360-MP3D-VO) publicly available, along with the source codes.


==> table_src/exp_scenes_test.tex <==
\begin{table*}[t!]
% \footnotesize
\fontsize{10}{15}\selectfont
\caption{\small{Experiments in synthetic scenes.}}
\label{tab:exp_scenes_test}

\begin{adjustbox}{max width=\textwidth}
\centering
\begin{tabular}{ c | c | cc | ccc | cc | ccc}

\hline
\hline

% First header
\multicolumn{2}{c}{} &
\multicolumn{5}{c}{\textbf{Rotation error $\times 10^{-3}$}} &
\multicolumn{5}{c}{\textbf{Translation error $\times 10^{-3}$}} \\
\cline{3-12}

% Second header
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{8-PA~\cite{higgins1981computer}} &
\multicolumn{1}{c}{\textbf{Ours-\eqref{eq:LM_SK}}} &
\multicolumn{1}{c}{GSM~\cite{pagani2011_sfm_some_loss_func}} &
\multicolumn{1}{c}{\eqref{eq:LM_SK_wRT}-$\omega(\epsilon_{\xi})$} &
\multicolumn{1}{c}{\textbf{Ours-\eqref{eq:LM_SK_wRT}-$\omega(\epsilon_{KS})$}} &
\multicolumn{1}{c}{8-PA~\cite{higgins1981computer}} &
\multicolumn{1}{c}{\textbf{Ours-\eqref{eq:LM_SK}}} &
\multicolumn{1}{c}{GSM~\cite{pagani2011_sfm_some_loss_func}} &
\multicolumn{1}{c}{\eqref{eq:LM_SK_wRT}-$\omega(\epsilon_{\xi})$} &
\multicolumn{1}{c}{\textbf{Ours-\eqref{eq:LM_SK_wRT}-$\omega(\epsilon_{KS})$}} \\
\hline

% MP3D-VO (0)
\multirow{3}{*}{MP3D-VO (0)} 
& Q75 & 
24.835 & \textbf{20.492} & 16.402 & 10.670 & \textbf{8.496} & 102.411 & \textbf{73.924} & 50.213 & 35.530 & \textbf{22.919} \\

& Q50 & 
11.473 & \textbf{10.097} & 7.790  & 3.641  & \textbf{3.272} & 38.752  & \textbf{30.020} & 21.287 & 10.465 & \textbf{8.596} \\

& Q25 & 
5.176  & \textbf{4.643}  & 3.598  & 1.658  & \textbf{1.582} & 15.116  & \textbf{13.001} & 9.406  & 5.455 & \textbf{5.010} \\
\hline

% MP3D-VO (1)
\multirow{3}{*}{MP3D-VO (1)} 
& Q75 & 
23.577 & \textbf{20.504} & 15.286 & 9.909 & \textbf{7.964} & 91.442 & \textbf{72.693} & 43.707 & 29.945 & \textbf{20.653} \\

& Q50 & 
10.827 & \textbf{9.515}  & 7.389  & 3.523 & \textbf{3.072} & 36.814 & \textbf{29.645} & 19.453 & 9.985  & \textbf{7.966}  \\

& Q25 & 
4.624  & \textbf{4.075}  & 3.277  & 1.638 & \textbf{1.524} & 14.745 & \textbf{12.276} & 8.501  & 4.611  & \textbf{4.009} \\
\hline

% TUM-VI
\multirow{3}{*}{TUM-VI} 
& Q75 &
44.479 & \textbf{40.514} & 49.291 & 39.938 & \textbf{38.256} & 221.131 & \textbf{199.042} & 166.594 & 169.122 & \textbf{140.846} \\

& Q50 &
27.211 & \textbf{24.969} & 27.226 & 21.075 & \textbf{19.241} & 117.701 & \textbf{104.742} & 82.457  & 74.661  & \textbf{62.743}  \\

& Q25 &
15.512 & \textbf{14.462} & 14.595 & 10.507 & \textbf{9.708}  & 58.791  & \textbf{53.283} & 40.899  & 33.724  & \textbf{28.800}  \\
\hline
\hline

\end{tabular}
\end{adjustbox}

\end{table*}

==> table_src/exp_threshold_test.tex <==
\begin{table*}[h!]
% \footnotesize
\fontsize{10}{15}\selectfont
\caption{\small{Experiments in synthetic scenes.}}
\label{tab:exp_threshold_test}

\begin{center}
\begin{tabular}{ c | c | c | c | c | c | c | c }

\hline
\hline

% Header
\multicolumn{2}{c}{} &
\multicolumn{1}{c}{\textbf{Rotation error}} &
\multicolumn{1}{c}{\textbf{Translation error}} &
\multicolumn{1}{c}{\textbf{Residual}} &
\multicolumn{1}{c}{\textbf{Iteration}} &
\multicolumn{1}{c}{\textbf{Time}} &
\multicolumn{1}{c}{\textbf{Outliers(\%)}} \\
\hline


% Rows

% Threshold 1
\multirow{5}{*}{Threshold 1} & 8-PA~\cite{higgins1981computer} \\
& GSM~\cite{pagani2011_sfm_some_loss_func} \\
& $\omega_{\xi}~\epsilon(\xi)$ \\
& $\epsilon(K, S)$ \\
& $\omega_{KS}~\epsilon(\xi)$ \\
\hline

% Threshold 2
\multirow{5}{*}{Threshold 2} & 8-PA \\
& GSM \\
& $\omega_{\xi}~\epsilon(\xi)$ \\
& $\epsilon(K, S)$ \\
& $\omega_{KS}~\epsilon(\xi)$ \\
\hline


\end{tabular}
\end{center}
\end{table*}
